A Dual-Path Model With Adaptive Attention For Vehicle Re-Identification

In recent years, attention models have been extensively used for person and vehicle re-identification. Most re-identification methods are designed to focus attention on key-point locations. However, depending on the orientation, the contribution of each key-point varies. In this paper, we present a novel dual-path adaptive attention model for vehicle re-identification (AAVER). The global appearance path captures macroscopic vehicle features while the orientation conditioned part appearance path learns to capture localized discriminative features by focusing attention on the most informative key-points. Through extensive experimentation, we show that the proposed AAVER method is able to accurately re-identify vehicles in unconstrained scenarios, yielding state of the art results on the challenging dataset VeRi-776. As a byproduct, the proposed system is also able to accurately predict vehicle key-points and shows an improvement of more than 7% over state of the art. The code for key-point estimation model is available at https://github.com/Pirazh/Vehicle_Key_Point_Orientation_Estimation.

==> amit.tex <==
\section{dnnrnprneprne}





==> neehar.tex <==
%\subsection{Network and Implementation Details}
%We first train the global appearance model, which is inspired by the work of Ranjan \textit{et.al.} \cite{ranjan2017l2} for face verification. The $L_2$ softmax loss function has been shown to significantly improve identity separation on large gallery sets. In experiments, we also refer this model as the baseline model. This baseline model, composed of ResNet101 backbone, is first pre-trained on ImageNet, and is later fine-tuned on several data sets, including Vehicle-ID and VeRi-776. 



%The $L_2$ softmax loss increases the intra-class cosine distances, improving classification and re-identification results. Specifically, the $L_2$ softmax loss maximizes the cosine similarity of two images of the same class and minimizes the cosine similarity of two images of different classes. 

%\subsection{Network Architecture}
%The baseline model consists of a ResNet-101 pre-trained on ImageNet followed by several linear layers. The fully connected layers of the ImageNet model are removed and replaced by four sequential fully connected layers. The [B x 2048] extracted features are passed through two linear layers of size [B x 2048] before being reduced by a third linear layer to a [B x 512] feature vector where B represents the batch size. Experimental data shows that feature vectors of size [B x 512] produce the most discriminating features. The fourth FC layer serves as a classifier to transform [B x 512] to [B x C] where B is the batch size and C is the number of classes. 

%\subsection{Baseline Network Training}
%The baseline model is only trained on one data set before being evaluated. Through experimentation, we have found that the network converges fastest when the $\alpha$ scaling parameter is learned by the network. Lastly, we have found that the network is highly sensitive to the $\alpha$ scaling parameters. 

%The ResNet-101 model is taken from the PyTorch torchvision library, and is trained with an initial learning rate of $1e^{-3}$, weight decay of ${5e^-4}$, momentum of 0.9, batch size of 64 and an initial $\alpha$ value of 40. The model is optimized using stochastic gradient descent with momentum. 


%The baseline model is able to achieve comparable performance to state-of-the-art models. This general appearance model achieves high accuracy without using local discriminating features, spatio-temporal information, or generated images to augment training data.

%The proposed pose-invariant model provides a significant improvement to baseline network performance on the VeRi-776 data set due to the data set's large variation in pose. Similarly, the proposed pose-invariant model provides minimal improvement on the Vehicle-ID data set due to the lack of variation in pose.



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{Figures/probe2.pdf}
        \caption{Probe Image}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn2_1.pdf}
        \caption{Top $1$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn2_2.pdf}
        \caption{Top $2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn2_3.pdf}
        \caption{Top $3$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn2_4.pdf}
        \caption{Top $4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn2_5.pdf}
        \caption{Top $5$}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn2_1.pdf}
        \caption{Top $1$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn2_2.pdf}
        \caption{Top $2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn2_3.pdf}
        \caption{Top $3$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn2_4.pdf}
        \caption{Top $4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn2_5.pdf}
        \caption{Top $5$}
    \end{subfigure}
    \caption{Comparison between Feature embedding of Baseline versus Proposed method in Veri 776 dataset; first row, sub figure a, is the probe image, second row, sub figures b to f, and the third row, sub figures g to k, are 5 returns of baseline model and proposed method with the highest similarity to the probe image.}
    \label{fig:baseline_VS_proposed_2}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{Figures/prob6.pdf}
        \caption{Probe Image}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/General_model_returns6_1.pdf}
        \caption{Top $1$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/General_model_returns6_2.pdf}
        \caption{Top $2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/General_model_returns6_3.pdf}
        \caption{Top $3$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/General_model_returns6_4.pdf}
        \caption{Top $4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/General_model_returns6_5.pdf}
        \caption{Top $5$}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/Part_model_returns6_1.pdf}
        \caption{Top $1$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/Part_model_returns6_2.pdf}
        \caption{Top $2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/Part_model_returns6_3.pdf}
        \caption{Top $3$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/Part_model_returns6_4.pdf}
        \caption{Top $4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/Part_model_returns6_5.pdf}
        \caption{Top $5$}
    \end{subfigure}
    \caption{Comparison between Feature embedding of Baseline versus Proposed method in Vehicle-ID; first row, sub figure a, is the probe image, second row, sub figures b to f, and the third row, sub figures g to k, are 5 returns of baseline model and proposed method with the highest similarity to the probe image.}
    \label{fig:baseline_VS_proposed_6}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.16\textwidth}
        \includegraphics[width=\textwidth]{Figures/probe1.pdf}
        \caption{Probe Image}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn1_1.pdf}
        \caption{Top $1$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn1_2.pdf}
        \caption{Top $2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn1_3.pdf}
        \caption{Top $3$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn1_4.pdf}
        \caption{Top $4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/GeneralReturn1_5.pdf}
        \caption{Top $5$}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn1_1.pdf}
        \caption{Top $1$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn1_2.pdf}
        \caption{Top $2$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn1_3.pdf}
        \caption{Top $3$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn1_4.pdf}
        \caption{Top $4$}
    \end{subfigure}
    \begin{subfigure}[b]{0.08\textwidth}
        \includegraphics[width=\textwidth]{Figures/PartReturn1_5.pdf}
        \caption{Top $5$}
    \end{subfigure}
    \caption{Comparison between Feature embedding of Baseline versus Proposed method in Veri 776 dataset; first row, sub figure a, is the probe image, second row, sub figures b to f, and the third row, sub figures g to k, are 5 returns of baseline model and proposed method with the highest similarity to the probe image.}
    \label{fig:baseline_VS_proposed_1}
\end{figure}

